The Higgs Mechanism with Diagrams: a didactic approach

We present a pedagogical treatment of the electroweak Higgs mechanism based solely on Feynman diagrams and S-matrix elements, without recourse to (gauge) symmetry arguments. Throughout, the emphasis is on Feynman rules and the Schwinger-Dyson equations; it is pointed out that particular care is needed in the treatment of tadpole diagrams and their symmetry factors.

==> SSB_Diagrams/Znewcommands.tex <==
\newcommand{\nc}{\newcommand}
\nc{\noi}{\noindent}
\newtheorem{opgave}{Excercise}
\nc{\bop}[1]{\begin{opgave}\begin{rm}{\bf#1} \newline\noi}
\nc{\eop}{\end{rm}\end{opgave}}
\nc{\dia}[1]{\mbox{{\Large{\bf diag}}}[#1]}
\nc{\diag}[3]{\raisebox{#3cm}{\epsfig{figure=diagrams/d#1.eps,width=#2cm}}}
%\nc{\diag}[3]{\dia{#1}}
\nc{\dg}[4]{\raisebox{#3cm}{\epsfig{figure=diagrams/album/#1.eps,width=#2cm}}\;\;\mbox{\small$#4$}\hspace{1cm}}
\nc{\dgs}[3]{\raisebox{#3cm}{\epsfig{figure=diagrams/album/#1.eps,width=#2cm}}}
\nc{\dgw}[3]{\raisebox{#3cm}{\epsfig{figure=diagrams/album/#1.eps,width=#2cm}}}
\nc{\bq}{\begin{equation}}
\nc{\eq}{\end{equation}}
\nc{\bqa}{\begin{eqnarray}} 
\nc{\eqa}{\end{eqnarray}}
\nc{\eqan}{\nonumber\end{eqnarray}}
\nc{\nl}{\nonumber \\}
\nc{\grf}{Green's function}
\nc{\grfs}{Green's functions}
\nc{\cgrf}{connected Green's function}
\nc{\cgrfs}{connected Green's functions}
\nc{\f}{\varphi}
\nc{\exb}[1]{\exp\!\left(#1\right)}
\nc{\avg}[1]{\left\langle #1\right\rangle}
\nc{\suml}{\sum\limits}
\nc{\prodl}{\prod\limits}
\nc{\intl}{\int\limits}
\nc{\ddv}[1]{{\partial\over\partial #1}}
\nc{\ddvv}[2]{{\partial^{#1}\over\left(\partial #2\right)^{#1}}}
\nc{\la}{\lambda}
\nc{\La}{\Lambda}
\nc{\eqn}[1]{Eq.(\ref{#1})}
\nc{\eqns}[1]{Eqs.(\ref{#1})}
\nc{\appndix}[3]{\section{{#2}\label{#3}}\input{#3}}
\nc{\cala}{{\cal A}}
\nc{\calb}{{\cal B}}
\nc{\cale}{{\cal E}}
\nc{\calr}{{\cal R}}
\nc{\calf}{{\cal F}}
\nc{\calh}{{\cal H}}
\nc{\calc}{{\cal C}}
\nc{\cald}{{\cal D}}
\nc{\calp}{{\cal P}}
\nc{\calt}{{\cal T}}
\nc{\calk}{{\cal K}}
\nc{\cals}{{\cal S}}
\nc{\caln}{{\cal N}}
\nc{\cali}{{\cal I}}
\nc{\calq}{{\cal Q}}
\nc{\calg}{{\cal G}}
%\nc{\calphi}{{\cal{\Phi}}}
\nc{\calphi}{\Psi}
\nc{\lra}{\;\leftrightarrow\;}
\nc{\stapel}[1]{\begin{tabular}{c} #1\end{tabular}}
\nc{\kolom}[1]{\left(\stapel{#1}\right)}
\nc{\al}{\alpha}
\nc{\be}{\beta}
\nc{\g}{\gamma}
\nc{\ga}{\gamma}
\nc{\Ga}{\Gamma}
\nc{\ka}{\kappa}
\nc{\om}{\omega}
\nc{\si}{\sigma}
\nc{\Si}{\Sigma}
\nc{\Sibar}{\overline{\Si}}
\nc{\ro}{\rho}
\nc{\tha}{\theta}
\nc{\ze}{\zeta}
\nc{\vph}{\vphantom{{A^A\over A_A}}}
\nc{\wph}{\vphantom{{A^A}}}
\nc{\order}[1]{{\cal O}\left(#1\right)}
\nc{\De}{\Delta}
\nc{\de}{\delta}
\nc{\vx}{\vec{x}}
\nc{\vxi}{\vec{\xi}}
\nc{\vy}{\vec{y}}
\nc{\vk}{\vec{k}}
\nc{\vn}{\vec{n}}
\nc{\vq}{\vec{q}}
\nc{\vp}{\vec{p}}
\nc{\vz}{\vec{z}}
\nc{\vt}{\vec{t}}
\nc{\nv}{\vec{n}}
\nc{\ve}{\vec{e}}
\nc{\vs}{\vec{s}}
\nc{\vr}{\vec{r}}
\nc{\hk}{\hat{k}}
\nc{\lijst}[1]{\begin{center}
  \fbox{\begin{minipage}{12cm}{#1}\end{minipage}}\end{center}}
\nc{\lijstx}[2]{\begin{center}
  \fbox{\begin{minipage}{#1cm}{#2}\end{minipage}}\end{center}}
\nc{\eps}{\epsilon}
\nc{\caput}[2]{\chapter{#1}\input{#2}}
\nc{\pd}{\partial}
\nc{\dtil}{\tilde{d}}
\nc{\vskp}{\vspace*{\baselineskip}}
\nc{\coos}{co\-ord\-in\-at\-es}
\nc{\calm}{{\cal{M}}}
\nc{\calj}{{\cal J}}
\nc{\call}{{\cal L}}
\nc{\calu}{{\cal U}}
\nc{\calw}{{\cal W}}
\nc{\msq}{\langle|\calm|^2\rangle}
\nc{\nsym}{F_{\mbox{{\tiny{symm}}}}}
\nc{\dm}[1]{\mbox{\bf dim}\!\left[#1\right]}
\nc{\fourv}[4]{\left(\begin{tabular}{c}
  $#1$\\$#2$\\$#3$\\$#4$\end{tabular}\right)}
\nc{\driev}[3]{\left(\begin{tabular}{c}
  $#1$\\$#2$\\$#3$\end{tabular}\right)}
\nc{\fs}[1]{/\!\!\!#1}
\nc{\dbar}[1]{{\overline{#1}}}
\nc{\tr}[1]{\mbox{Tr}\left(#1\right)}
\nc{\deter}[1]{\mbox{det}\left(#1\right)}
\nc{\row}[4]{$#1$ & $#2$ & $#3$ & $#4$}
\nc{\matv}[4]{\left(\begin{tabular}{cccc}
   #1 \\ #2 \\ #3 \\ #4\end{tabular}\right)}
\nc{\twov}[2]{\left(\begin{tabular}{cccc}
   $#1$ \\ $#2$\end{tabular}\right)}
\nc{\ubar}{\dbar{u}}
\nc{\vbar}{\dbar{v}}
\nc{\wbar}{\dbar{w}}
\nc{\lng}{longitudinal}
\nc{\pol}{polarisation}
\nc{\longpol}{\lng\ \pol}
\nc{\bnum}{\begin{enumerate}}
\nc{\enum}{\end{enumerate}}
\nc{\nubar}{\overline{\nu}}
\nc{\mau}{{m_{\mbox{{\tiny U}}}}}
\nc{\mad}{{m_{\mbox{{\tiny D}}}}}
\nc{\qu}{{Q_{\mbox{{\tiny U}}}}}
\nc{\qd}{{Q_{\mbox{{\tiny D}}}}}
\nc{\vau}{{v_{\mbox{{\tiny U}}}}}
\nc{\aau}{{a_{\mbox{{\tiny U}}}}}
\nc{\aad}{{a_{\mbox{{\tiny D}}}}}
\nc{\vad}{{v_{\mbox{{\tiny D}}}}}
\nc{\mw}{{m_{\mbox{{\tiny W}}}}}
\nc{\mt}{{m_{\mbox{{\tiny t}}}}}
\nc{\mv}{{m_{\mbox{{\tiny V}}}}}
\nc{\mz}{{m_{\mbox{{\tiny Z}}}}}
\nc{\mf}{{m_{\mbox{{\tiny f}}}}}
\nc{\gz}{{\Gamma_{\mbox{{\tiny Z}}}}}
\nc{\mh}{{m_{\mbox{{\tiny H}}}}}
\nc{\gw}{{g_{\mbox{{\tiny W}}}}}
\nc{\gs}{{g_{\mbox{{\small s}}}}}
\nc{\qw}{{Q_{\mbox{{\tiny W}}}}}
\nc{\qe}{{Q_{\mbox{{\tiny e}}}}}
\nc{\qc}{{Q_{\mbox{{\tiny c}}}}}
\nc{\law}{{\Lambda_{\mbox{{\tiny W}}}}}
\nc{\obar}{\overline}
\nc{\gfer}{G_{\mbox{{\tiny F}}}}
\nc{\guuh}{{g_{\mbox{{\tiny UUH}}}}}
\nc{\gtth}{{g_{\mbox{{\tiny ttH}}}}}
\nc{\gffh}{{g_{\mbox{{\tiny ffH}}}}}
\nc{\gwwz}{{g_{\mbox{{\tiny WWZ}}}}}
\nc{\gwwh}{{g_{\mbox{{\tiny WWH}}}}}
\nc{\gwwhh}{{g_{\mbox{{\tiny WWHH}}}}}
\nc{\gzzh}{{g_{\mbox{{\tiny ZZH}}}}}
\nc{\gvvh}{{g_{\mbox{{\tiny VVH}}}}}
\nc{\ghhh}{{g_{\mbox{{\tiny HHH}}}}}
\nc{\ghhhh}{{g_{\mbox{{\tiny HHHH}}}}}
\nc{\gzzhh}{{g_{\mbox{{\tiny ZZHH}}}}}
\nc{\thw}{\theta_W}
\nc{\sw}{{s_{\mbox{{\tiny W}}}}}
\nc{\cw}{{c_{\mbox{{\tiny W}}}}}
\nc{\ward}[2]{\left.#1\right\rfloor_{#2}}
\nc{\vpa}{(1+\g^5)}
\nc{\vma}{(1-\g^5)}
\nc{\gwzh}{{g_{\mbox{{\tiny WZH}}}}}
\nc{\gudh}{{g_{\mbox{{\tiny UDH}}}}}
\nc{\gwcj}{{g_{\mbox{{\tiny Wcj}}}}}
\nc{\gwcjg}{{g_{\mbox{{\tiny Wcj$\g$}}}}}
\nc{\gwwcc}{{g_{\mbox{{\tiny WWcc}}}}}
\nc{\gzcc}{{g_{\mbox{{\tiny Zcc}}}}}
\nc{\none}[1]{ }
\nc{\Vir}{{V_{\mbox{{\tiny IR}}}}}
\nc{\kt}[1]{\left|#1\right\rangle}
\nc{\br}[1]{\left\langle#1\right|}
\nc{\bak}[3]{\left\langle #1\!\left| #2 \right|\! #3\right\rangle}
\nc{\bk}[2]{\left\langle #1\right|\left.\!\!#2\right\rangle}
\nc{\tw}{\tilde{w}}
\nc{\hDe}{\nabla}
\nc{\bino}[2]{\left(\begin{tabular}{c}$#1$\\$#2$\end{tabular}\right)}
\nc{\Om}{\Omega}
\nc{\Omb}{\overline{\Omega}}
\nc{\qbar}{\bar{q}}
\nc{\leeg}[1]{}
\nc{\dilog}{\mbox{Li}_2}
%\nc{\marx}[1]{\marginpar{\fbox{{\bf E\,\ref{#1}}}}}
\nc{\marx}[1]{\marginpar{\fbox{\ref{#1}}}}
\nc{\ebar}{\bar{\eta}}
\nc{\eebar}{\eta\,\ebar}
\nc{\xibar}{\bar{\xi}}
\nc{\Sib}{\overline{\Si}}
\nc{\hw}{\hat{w}}
\nc{\cthe}{\cos\theta\;}
\nc{\sthe}{\sin\theta\;}
\nc{\ctthe}{\cos2\theta\;}
\nc{\stthe}{\sin2\theta\;}
\nc{\bmat}{\left(\begin{tabular}}
\nc{\emat}{\end{tabular}\right)}
\nc{\idx}[1]{\index{#1}#1}
\nc{\pars}{\partial_s}
\nc{\parv}{\partial_v}
\nc{\parw}{\partial_w}
\nc{\vv}{{\bf{v}}}
\nc{\vw}{{\bf{w}}}
\nc{\veps}{\vec{\eps}}
\nc{\vphi}{\vec{\phi}}
\nc{\fall}[2]{#1^{\underline #2}}
\nc{\sihad}{\si_{\mbox{{\tiny had}}}}
\nc{\dexy}{\de_{xy}}
\nc{\gotf}{\mathfrak{F}}
\nc{\gotm}{\mathfrak{m}}
\nc{\gf}{\mathfrak{f}}
\nc{\gh}{\mathfrak{h}}
\nc{\gc}{\mathfrak{c}}
\nc{\lagr}{{\mathfrak L}}
\nc{\gotc}{{\mathfrak C}}
\nc{\gotp}{{\mathfrak P}}
\nc{\got}{{\mathfrak T}}
\nc{\plaatje}[4]{\begin{figure}\begin{center}
  \includegraphics[width=#2cm]{#1}\caption{#3}\label{#4}\end{center}\end{figure}}
\nc{\figur}[1]{figure \ref{#1}}
\nc{\logbe}{\log\left({1+\be\over1-\be}\right)}
\nc{\calmlight}{\calm_{\mbox{\tiny{light}}}}
\nc{\calmlightcut}{\calm_{\mbox{\tiny{light,cut}}}}
\nc{\tinyf}{\begin{tiny}{\bf{\em F\/}}\end{tiny}}
\nc{\Veff}{V_{\mbox{{\tiny eff}}}}
\nc{\psibb}{\bar{\psi}}
\nc{\muh}{\hat{\mu}}
\nc{\lah}{\hat{\lambda}}
\nc{\uh}{\hat{u}}
\nc{\gow}{\mathfrak{W}}
\nc{\etp}{\eta_+}
\nc{\etm}{\eta_-}
\nc{\conto}{\mbox{{\Large $\leadsto$}}}
\nc{\sfc}[1]{\mbox{{\small ${#1}$}}}
\nc{\smf}{\mathfrak{sm}}
% \nc{\implies}{\;\Rightarrow\;}
\nc{\vf}{\vec{\phi}}
\nc{\chib}{\bar{\chi}}
\nc{\vchi}{\vec{\chi}}
\nc{\vchib}{\vec{\chib}}
\nc{\hmu}{\hat{\mu}}
\nc{\hu}{\hat{u}}
\nc{\hal}{\hat{\al}}
\nc{\ran}{\mathfrak{r}()}
\nc{\vell}{\vec{\ell}}
\nc{\mtil}{\tilde{m}}
\nc{\msbar}{$\overline{\mbox{MS}}$}
\nc{\half}{\mbox{{\small${1\over2}$}}}
\nc{\drhalf}{\mbox{{\small${3\over2}$}}}
\nc{\kwart}{\mbox{{\small${1\over4}$}}}
\nc{\fc}{\phi_c}
\nc{\Pigg}{\Pi_{\g\g}}
\nc{\Piv}{\Pi_{\mbox{{\tiny V}}}}
\nc{\gt}{\mathfrak{t}}
\nc{\gn}{\mathfrak{n}}
\nc{\va}{\vec{a}}
\nc{\vb}{\vec{b}}
\nc{\vc}{\vec{c}}
\nc{\vd}{\vec{d}}
\nc{\vsi}{\vec{\si}}
\nc{\must}{\stackrel{\downarrow}{=}}
\nc{\vreps}{\varepsilon}
\nc{\cth}{c_\theta}
\nc{\sth}{s_\theta}
\nc{\da}{{\dot{a}}}
\nc{\db}{{\dot{b}}}
\nc{\dc}{{\dot{c}}}
\nc{\dd}{{\dot{d}}}
\nc{\dee}{{\dot{e}}}
\nc{\nosum}{\mbox{(no summation)}}
%\nc{\Bbar}{\overline{B}}
\nc{\Bbar}{{B}}
\nc{\one}{{\bf 1}}
\nc{\hA}{\hat{A}}
\nc{\hB}{\hat{B}}





